A Theoretical Framework for the Electrochemical Characterization of Anisotropic Micro-Emulsions

Micro emulsions (MEs) offer an exceptionally broad spectrum of applications covering sensing, electrosynthesis, supercapacitors and redox-flow batteries. Herein, we develop the theory for a sophisticated electrochemical characterizion of MEs with a spatially and time-invariant anisotropy in the diffusion domain by means of cyclic voltammerty (CV). By introducing spatially dependent diffusion coefficients into Ficks' first law, we derive a modified diffusion equation to simulate any inherent anisotropy of the ME under investigation. Moreover, by formulating an extended second-order homogeneous six-member square scheme for a kinetically controlled two-step two-electron reaction we capture the intricate entanglement of chemical and electrochemical equilibria. Our theoretical concept is finally validated by experimental CV data for the ME based two-step redox reaction of methyl-viologen which paves the way for a quantitative electrochemical characterization MEs.

==> 03_Keywords.tex <==
Micro-Emulsions; Redox-Flow Batteries; Two-Electron Transfer; Methyl-Viologen; E\textsubscript{k}E\textsubscript{k}-Mechanism

